Multiple Analyses, Requirements Once: simplifying testing & verification in automotive model-based development

In industrial model-based development (MBD) frameworks, requirements are typically specified informally using textual descriptions. To enable the application of formal methods, these specifications need to be formalized in the input languages of all formal tools that should be applied to analyse the models at different development levels. In this paper we propose a unified approach for the computer-assisted formal specification of requirements and their fully automated translation into the specification languages of different verification tools. We consider a two-stage MBD scenario where first Simulink models are developed from which executable code is generated automatically. We (i) propose a specification language and a prototypical tool for the formal but still textual specification of requirements, (ii) show how these requirements can be translated automatically into the input languages of Simulink Design Verifier for verification of Simulink models and BTC EmbeddedValidator for source code verification, and (iii) show how our unified framework enables besides automated formal verification also the automated generation of test cases.

==> chapters/caseStudies.tex <==
%\paragraph{Driveline State Request and E-Clutch Control.}
\paragraph{R\&D Prototype Features.}
Our case study was conducted using the auto-generated code of three R\&D prototype Simulink models: a model of the next-gen \emph{Driveline State Request} (DSR) feature, of the next-gen \emph{E-Clutch Control} (ECC) feature and of the next-gen \emph{Low Speed Control for Parking} (LSC) feature. 
None of these features are safety-critical.
Let us describe the role and importance of these three features.
Energy saving, exhaust emission reduction, and exhaust noise reduction are among the main objectives in the development of modern vehicles. 
On flat roads, the engine drag torque typically slows down the vehicle when the driver takes his foot from the accelerator pedal. 
A vehicle with a combustion engine can be operated in Sailing Mode when the vehicle is rolling without engine drag torque in order to maintain its speed and to save fuel in certain driving situations and where the driver is not actively accelerating or braking the vehicle. 
In Sailing Mode, the driveline\footnote{A motor vehicle's driveline consists of the parts of the powertrain excluding the engine. It is the portion of a vehicle, after the prime mover, that changes depending on whether a vehicle is front-wheel, rear-wheel, or four-wheel drive.} is opened automatically when the driver releases the accelerator pedal. 
When the driveline is open, the engine can be shut off or run at idle speed without introducing drag torque in order to reduce fuel consumption. 
Different system- or driver-interactions, such as pressing the brake or accelerator pedal, will result in closing the driveline again. 
The DSR feature implements the decision logic to open or close the driveline. 
This feature takes driver interactions and vehicle status information to decide in which situations the driveline should be opened and closed again. 
The ECC feature calculates the desired clutch torque capacity and corresponding engine control torques or speeds for opening and closing the driveline.
Different from these two, the LSC feature allows the vehicle to park automatically and operates at relatively low speeds compared to other driving situations. 
During assisted parking maneuvers, the vehicle speed has to be controlled at low vehicle speed targets and scenarios like climbing on a curb during parking have to be supported. The selected feature Low Speed Control takes the vehicle speed set point from Park Assist and controls the combustion engine speed and the brakes during automated parking.

% 
%% The majority of all requirements specify invariant properties ($132$ requirements) 
%% and only include a total of $6$ response properties.
%%
\begin{table}[t]
\centering
\caption{The variables and calibration parameters of the Simulink models.}
{\small
\begin{tabular}{l r|c|c|c|c|c|c|}
	\cline{3-8}
	& & \multicolumn{3}{c|}{Scalar} & \multicolumn{3}{c|}{Array/Matrix} \\
	\cline{3-8}
	& & bool & int & float & bool & int & float\\
	\hline \hline
	\multicolumn{1}{|c|}{\multirow{2}{*}{DSR}} & I/O Vars & $7$ & $16$ & $8$ & $0$ & $1$ ($1{\times}10$) & 1 ($1{\times}10$) \\
	\cline{2-8}
	\multicolumn{1}{|c|}{} & Calibration Pars & $15$ & $3$ & $24$ & 1 ($1{\times}12$) & 1 ($1{\times}32$) & 9 ($1{\times}6 \dots 12$) \\ 
	\hline \hline
	\multicolumn{1}{|c|}{\multirow{2}{*}{ECC}} & I/O Vars & $3$ & $4$ & $29$ & $0$ & $0$ & $0$ \\
	\cline{2-8}
	\multicolumn{1}{|c|}{} & Calibration Pars & $7$ & $1$ & $71$ & $0$ & $0$ & 72 ($1 {\times} 2 \dots 11 {\times} 11$) \\
	 \hline
	 \multicolumn{1}{|c|}{\multirow{2}{*}{LSC}} & I/O Vars & $5$ & $12$ & $14$ & $0$ & $0$ & $0$ \\
	 \cline{2-8}
	 \multicolumn{1}{|c|}{} & Calibration Pars & $2$ & $0$ & $50$ & $0$ & $0$ & 17 ($1 {\times} 7 \dots 14$) \\
	\hline
\end{tabular}
}
\label{table:vars_and_cal_pars}
\end{table}
%\vspace{-1em}
 
%\paragraph{Model Characteristics.}
%The Simulink model for the DSR feature has $42$ functional requirements, $28$ inputs, six outputs, $53$ calibration parameters and $1149$ blocks.
%Calibratable parameters remain constant during software execution but can be 
%adjusted before the execution for tuning or selecting the possible 
%functionalities. 
%Calibration is the adjustment of calibratable parameters of software functions realizing the control functionalities.
%This model contains several variables as summarized in the first two rows of Table~\ref{table:vars_and_cal_pars}.
%The C code comprises about $2100$ lines. 
%The next-gen DSR feature has several calibration parameters, amongst others $42$ scalar 
%parameters and nine array parameters of six to $12$ single-precision floating-point elements, one Boolean array with $12$ elements and one unsigned 8-bit integer array with $32$ elements. 
%
%The Simulink model for the ECC feature has $70$ functional requirements, $27$ inputs, nine outputs, 151 calibration parameters and 2098 blocks.
%In total, it comprises about $4900$ lines of C code. 
%This model contains Boolean, integer and a huge number of floating-point variables, see Table~\ref{table:vars_and_cal_pars}.
%The calibration parameters include 79 scalar parameters and 13 arrays of single-precision floats. 
%
%The Simulink model for the LSC feature has $41$ functional requirements, 26 inputs, 5 outputs, 69 calibration parameters and 1095blocks ($\approx 1500$ lines of C code). 
%All input and output signals are scalar with the following data type distribution: 5 Boolean, 12 unsigned 8-bit integer and 14 single-precision floating point. 
%Among the calibration parameters we have 52 scalar (2 Boolean and 50 single-precision floating-point) parameters and 17 parameters are arrays with 7 to 14 single-precision floating-point elements.

% DSR: 50 INV, 4 N Step Delays
% ECC: 82 INV, 2 N Step Delays
\paragraph*{Requirement Characteristics.}
For the DSR case study, from $42$ functional requirements we extracted $54$ properties, consisting of 50 invariants and four bounded-response properties.
Invariant properties are assertions that are supposed to hold for all reachable states.
Bounded-response properties request that a certain assertion holds within a given number of computational steps whenever a given, second assertion holds.
For the ECC case study, from $70$ functional requirements we extracted $82$ invariants and two bounded-response properties.

TODO: Missing numbers for LSC!
% TODO: Missing numbers for LSC!


==> images/scopes/globally.tex <==
\begin{tikzpicture}
	% timeline
	\draw[-] (0,0) -- (10,0);
	% Small tickmarks on the x axis
	\foreach \x in {0,0.5,...,10} {
			\draw (\x, 0.1) -- (\x, -0.1);
	}
	%big ticks at the beginning and end of axis
	\draw[thick] ( 0, 0.2) -- ( 0, -0.2);
	\node at ( 0, -0.5) {$0$};
	\draw[thick] (10, 0.2) -- (10, -0.2);
	\node at (10, -0.5) {$T$};
	
	%globally
	\draw[-, black25, fill] (0,0.5) -- (0, 0.8) -- (10, 0.8) -- (10,0.5) -- (0,0.5);
\end{tikzpicture}


==> images/scopes/initially.tex <==
\begin{tikzpicture}
	% timeline
	\draw[-] (0,0) -- (10,0);
	% Small tickmarks on the x axis
	\foreach \x in {0,0.5,...,10} {
			\draw (\x, 0.1) -- (\x, -0.1);
	}
	%big ticks at the beginning and end of axis
	\draw[thick] ( 0, 0.2) -- ( 0, -0.2);
	\node at ( 0, -0.5) {$0$};
	\draw[thick] (10, 0.2) -- (10, -0.2);
	\node at (10, -0.5) {$T$};
	
	%globally
	\draw[-, black25, fill] (0,0.5) -- (0, 0.8) -- (0.4, 0.8) -- (0.4,0.5) -- (0,0.5);
\end{tikzpicture}

